Bridging the Reproducibility Divide: Open Source Software's Role in Standardizing Healthcare AI

Our analysis of recent AI4H publications reveals that, despite a trend toward utilizing open datasets and sharing modeling code, 74% of AI4H papers still rely on private datasets or do not share their code. This is especially concerning in healthcare applications, where trust is essential. Furthermore, inconsistent and poorly documented data preprocessing pipelines result in variable model performance reports, even for identical tasks and datasets, making it challenging to evaluate the true effectiveness of AI models. Despite the challenges posed by the reproducibility crisis, addressing these issues through open practices offers substantial benefits. For instance, while the reproducibility mandate adds extra effort to research and publication, it significantly enhances the impact of the work. Our analysis shows that papers that used both public datasets and shared code received, on average, 110% more citations than those that do neither--more than doubling the citation count. Given the clear benefits of enhancing reproducibility, it is imperative for the AI4H community to take concrete steps to overcome existing barriers. The community should promote open science practices, establish standardized guidelines for data preprocessing, and develop robust benchmarks. Tackling these challenges through open-source development can improve reproducibility, which is essential for ensuring that AI models are safe, effective, and beneficial for patient care. This approach will help build more trustworthy AI systems that can be integrated into healthcare settings, ultimately contributing to better patient outcomes and advancing the field of medicine.

==> sections/abstract.tex <==
Artificial intelligence for healthcare (AI4H) has significant health, ethical, and legal implications due to its direct impact on human lives. However, the field is facing a reproducibility crisis that raises concerns about the deployment of AI4H systems.
% Key barriers include private datasets, proprietary code, and the lack of standardized data preprocessing pipelines.
Our analysis of recent AI4H publications reveals that, despite a trend toward utilizing open datasets and sharing modeling code, 74\% of AI4H papers still rely on private datasets or do not share their code. This is especially concerning in healthcare applications, where trust is essential. Furthermore, inconsistent and poorly documented data preprocessing pipelines result in variable model performance reports, even for identical tasks and datasets, making it challenging to evaluate the true effectiveness of AI models.

% While reproducibility mandate does add more effort to publications, it is likely to enhance their impact.
\rev{Despite the challenges posed by the reproducibility crisis, addressing these issues through open practices offers substantial benefits.} For instance, while the reproducibility mandate adds extra effort to research and publication, it significantly enhances the impact of the work. Our analysis shows that papers that used both public datasets and shared code received, on average, 110\% more citations than those that do neither—more than doubling the citation count.

\rev{Given the clear benefits of enhancing reproducibility, it is imperative for the AI4H community to take concrete steps to overcome existing barriers.} The community should promote open science practices, establish standardized guidelines for data preprocessing, and develop robust benchmarks. Tackling these challenges through open-source development can improve reproducibility, which is essential for ensuring that AI models are safe, effective, and beneficial for patient care. This approach will help build more trustworthy AI systems that can be integrated into healthcare settings, ultimately contributing to better patient outcomes and advancing the field of medicine.

==> sections/critiques.tex <==
\section{ML4H Review Summarized}
\begin{enumerate}
    \item Structure and Organization:
    \begin{itemize}
        \item Suggestion to move Appendix B into the main discussion section (Straightforward, and easy) (done)
        \item Recommendation to improve the standardization section with more analysis (hard)
        \item Request to move Table 1 within formatting constraints (not needed)
    \end{itemize}

    \item Methodology Concerns: (Maybe more abstract details or supplementary details).
    \begin{itemize}
        \item Critique of weak methodology, particularly regarding initial filtering and keyword search (implemented validation set Table to quantify for n=30 papers)
        \item Request for clarification on selection criteria for conferences and papers (Added)
        \item Questions about time criteria for paper selection (Done) 
        \item Concern about insufficient analysis of widely adopted tools (Done)
    \end{itemize}

    \item Data and Analysis:
    \begin{itemize}
        % \item Request for total number of papers scraped and included (Resolveable)
        \item Suggestion to analyze data-use agreements and pseudo-code (hard)
        \item Request for analysis of code sharing and public datasets across different tasks (resolved)
        \item Critique of inconclusive results, particularly regarding Figure 1 (resolved in new)
    \end{itemize}

    \item Clarity and Specificity:
    \begin{itemize}
        \item Request for clarification on what transparency refers to (resolveable/trivial)
        \item Suggestion to include a summary of correct standardized high-level steps (resolveable, but also trivial)
        \item Concern about the potential dangers of standardized dataset processing (resolved/trivial)
    \end{itemize}

    \item Reproducibility and Standardization:
    \begin{itemize}
        \item Emphasis on the importance of standardization in healthcare AI research
        \item Discussion of the challenges in tracking open-source tool usage (Discuss GitHub Stars, Citation Counts with limitations)
        \item Debate on the benefits of standardized open-source dataset benchmarks (questionable?)
    \end{itemize}

    % \item Future Improvements:
    % \begin{itemize}
    %     \item Plans to expand literature search and conduct small studies on reproducibility
    %     \item Exploration of using large language models for better contextualization
    %     \item Proposal to develop a composite metric for tool usage and community interest
    % \end{itemize}
\end{enumerate}

==> sections/reproducibility_crisis.tex <==
\section{Introduction} 
AI models are increasingly used in healthcare for tasks such as disease diagnosis, drug recommendation, medical coding, report generation, and mortality prediction \cite{Habehh2021-tn_MLHC_survey}. However, improper validation and deployment of these models can lead to severe consequences, ranging from inadequate coverage of patients \rev{\cite{mittermaier2023bias_in_medical_AI}} to legal challenges \rev{\cite{napolitano_2023_health_insur_lawsuit, vcartolovni2022ethical_legal_considerations_review}}. 
The FDA's regulatory framework for AI/ML-based Software as a Medical Device (SaMD) has approved over 500 AI-enabled medical devices as of 2024, with the approval process heavily emphasizing model validation and reproducibility \cite{Center-for-Devices2024-zp}. The FDA's {\it predetermined change control plan} specifically requires manufacturers to demonstrate evidence-based and transparent approaches with reproducible model performance~\cite{Center-for-Devices2023-ee}.
Given the high-stakes nature of healthcare \cite{10.1371/journal.pmed.0020124_whymostresearchfalse}, validating and reproducing research findings is crucial not only for advancing state-of-the-art research in AI4H but also for ensuring the safe deployment of these models in clinical practice.

This paper aims to define reproducibility in the context of AI4H \rev{in 2024}, describe its research landscape, and propose practical steps to address the reproducibility challenges and improve transparency. \rev{To the best of our knowledge, our study presents the first large-scale analysis of reproducibility in AI4H as of 2024, examining thousands of papers. While \cite{mcdermott2019reproducibilitymachinelearninghealthcrisis} provides a highly detailed analysis of AI4H in 2018, our work expands the scope by an order of magnitude and introduces an automated approach to assess reproducibility, which is particularly valuable given the significant increase in the number of AI4H publications. Unlike general AI domains studied in prior reproducibility work \cite{gundersen2018reproducible_call, hutson2018artificial_crisis_review_call}, healthcare presents distinct challenges with its high-stakes outcomes, privacy constraints, and need for domain expertise. Furthermore, our analysis incorporates additional metrics such as citation patterns and research topics to demonstrate the tangible benefits of enhancing reproducibility. As the AI4H field has expanded tremendously in the past five years \cite{senthil2024bibliometric_trends_AI4H}, we believe it is critical for another review of the state of reproducibility in AI4H.}

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{figs/ScrapingPipeline.drawio.png}
    \caption{Paper Data Collection and Analysis: (a) Paper scraping details: We scrape PDF files directly from conference webpages, extracting and cleaning important paper details like title, authors, abstracts, and emails. We query BioC to scrape paper information from PubMed\rev{'s Open Access Database}, related to research papers that contain the terms AI, deep learning, machine learning, healthcare, electronic health records, and electronic medical records into XML formats. (b) Stacked bar chart of total number of papers scraped each year, showing a steady increase in paper counts over time. (c) Key analyses performed: Mapping citation counts to each paper using scholarly services like SerpAPI \cite{serpapi2024}, Semantic Scholar \cite{Kinney2023TheSS_Semantic_scholar}, and PMIDcite \cite{gusenbauer2020academic_pmid_cite}; scraping affiliation details by classifying emails or affiliations sourced from PubMed's MEDLINE API \cite{gusenbauer2020academic_pmid_cite}; classifying each paper's topic by its abstract and title with a medically fine-tuned large language model (OpenBioLLM-70b); checking for code sharing by identifying specific code keywords (e.g., GitHub, Zenodo, Colab, GitLab) in each paper's main text \rev{(excluding the references)}; assessing public dataset usage by checking for famous dataset keywords in the main text and cross-referencing each paper with the PapersWithCode API. We go into further detail in Appendix \ref{apd: Methodology Details}.}
    % \vspace{-0.6cm}
    \label{fig:scraping}
\end{figure}

% \subsection{Definition of Reproducibility in AI4H}
\subsection{\rev{Technical Reproducibility Is a Cornerstone in AI4H}}
Reproducibility, due to its multi-faceted nature, encompasses a variety of definitions across different fields \cite{desai2024reproducibilityartificialintelligencemachine_definition, NAP25303_Broad_definitions_reproducibility}. In computer science, the Association for Computing Machinery (ACM) defines reproducibility as the ability of a different team to obtain the same results using the same experimental setup (i.e., code, data, and methodological specifics) \cite{semmelrock2023reproducibilitymachinelearningdrivenresearch}.  In the AI4H domain, McDermott et al. \cite{mcdermott2019reproducibilitymachinelearninghealthcrisis} further delineates reproducibility into three sub-categories:
\begin{enumerate}
    \item {\bf Technical reproducibility:} {\it Can results be reproduced under technically identical conditions?} 
    This involves reproducing the precise results reported in a study using the same code and dataset.
    \item {\bf Statistical reproducibility:} {\it Can results be reproduced under statistically identical conditions?} 
     This refers to reproducing statistically equivalent results when using resampled data or random seeds.
    \item {\bf Conceptual reproducibility:} {\it Can results be reproduced under conceptually identical conditions?} 
    This involves generalizing the study’s claims to new but conceptually identical settings (e.g., similar datasets, models, or tasks).
\end{enumerate}

\rev{The relationship between technical, statistical, and conceptual reproducibility in AI for healthcare is complex and multifaceted. Research has demonstrated that achieving technical reproducibility does not guarantee conceptual reproducibility, and furthermore, that conceptual reproducibility itself may be an inherently ambiguous and unnecessary objective. For instance, \cite{futoma2020myth_of_generalisability} presents a compelling argument that models can provide significant value even when their effectiveness is limited to specific patient populations. This perspective challenges the notion that broad generalizability is always necessary for clinical utility. In a related investigation, \cite{zech2018variable_generalisability} conducted an extensive study of deep learning models across diverse patient cohorts and healthcare systems. Their findings revealed that model performance is intrinsically linked to the characteristics of the training data distribution, and notably, that attempts to train models across multiple cohorts often result in the models inadvertently learning to exploit confounding variables - such as the originating hospital system - rather than clinically relevant features within medical imaging data. This phenomenon underscores the complexity of achieving true generalizability. Furthermore, in the domain of causal machine learning, performance heterogeneity across different populations is not viewed as a limitation but rather as a fundamental aspect of understanding treatment effects \cite{feuerriegel2024causal_ML}.}

\rev{While these meta-analyses \cite{futoma2020myth_of_generalisability, zech2018variable_generalisability, feuerriegel2024causal_ML} present varying perspectives on conceptual reproducibility, they all implicitly depend on a foundation of technical reproducibility. The ability to replicate experiments and validate results across different patient populations serves as a crucial prerequisite for understanding how model performance varies across heterogeneous conditions. Without access to the underlying code and data, meaningful investigation of how new frontier AI models perform in diverse clinical contexts becomes virtually impossible. Moreover, the absence of technical reproducibility prevents direct verification of reported findings. This highlights a fundamental issue: while conceptual reproducibility or generalizability may neither be achievable nor necessary in all cases, technical reproducibility remains essential for rigorously examining and auditing claims about model performance and generalizability. Unfortunately, as illustrated in Figures \ref{fig:code_trends} and \ref{fig:data_trends}, achieving technical reproducibility continues to be a significant obstacle in the field of AI for healthcare.}

\rev{Thus, t}his paper primarily focuses on the \textbf{technical reproducibility}, as it serves as a prerequisite to experimentally validating the statistical and conceptual reproducibility and is surprisingly a largely unresolved issue in the AI4H domain.

% \subsection{Reproducibility Landscape in AI4H}
\section{The AI4H Reproducibility Crisis} \label{sec: Crisis}
To better understand the current reproducibility landscape, we scraped \rev{528} papers from three major AI4H conferences, Conference on Health, Inference, and Learning (CHIL), Machine Learning for Health Symposium (ML4H), and Machine Learning for Healthcare (MLHC), as well as \rev{2,082} PubMed papers filtered by whether their manuscripts contained mentions of AI and healthcare from 2018 to 2024 (see Appendix for the detailed search query), as shown in Figure \ref{fig:scraping}. We investigated various aspects of technical reproducibility, such as public dataset usage and code sharing. 

We identify three key reproducibility challenges that \rev{uniquely} persist in the AI4H domain:
\begin{enumerate}
\item \textbf{Private datasets:} Healthcare data's sensitive nature often necessitates the use of private datasets, preventing direct result replication by other researchers.
% This is particularly challenging in healthcare, where privacy regulations tightly control access to high-quality patient data.
\item \textbf{Proprietary code:} Many AI4H models use proprietary algorithms, hindering transparency and reproducibility. 
% Without access to the underlying code or detailed descriptions of model architectures and hyperparameters, replicating results or assessing model validity becomes nearly impossible.
\item \textbf{Lack of standardization in data processing:} Even when datasets and code are available, the absence of standardized preprocessing practices leads to significant variability in reported outcomes. 
% This inconsistency complicates result comparison across different studies, undermining the field's progress.
\end{enumerate}

\subsection{Private Datasets}
\begin{figure}[t]
    \centering
\includegraphics[width=1.0\linewidth]{figs/DatasetReproducibility.drawio.png}
    \caption{Trends in Public Dataset Usage: (a) Distribution of public dataset usage over time and across venues: MIMIC is the most commonly used or mentioned public dataset; private datasets dominate overall each year; conferences use more public datasets than journal papers. (b) Rate of public dataset usage across topics: Biosignal papers use the most public datasets. (c) Rate of public dataset usage across affiliations: Industry surprisingly uses the most public datasets. (d) Distribution of public dataset usage over time: Papers using public datasets have higher citation counts on average every year. The maximum number of citations on the y-axis is capped at 50 to focus on non-outlier behavior. (e) Cumulative distribution of using public datasets: Papers that use public datasets tend to have greater citation counts, regardless of outlier status.}
    % \vspace{}
    \label{fig:data_trends}
\end{figure}

Private datasets pose a major obstacle to reproducibility in AI4H. Patient confidentiality and regulations like the Health Insurance Portability and Accountability Act (HIPAA) severely restrict access to raw patient data, preventing researchers from sharing datasets used in AI model development. These limitations make it nearly impossible to verify results from models trained on private data, such as Google's breast cancer detection model \cite{McKinney2020_google_breast_cancer_detection}. This is particularly concerning when models claim to outperform human experts. Furthermore, the variability in healthcare data across institutions and regions exacerbates the challenge of developing generalizable models.

Proposed alternatives have significant drawbacks. Synthetic datasets often lack the complexity of real patient data, omitting rare diseases, unique treatment combinations, and intricate demographic-health interactions. This can result in models that perform well in controlled settings but fail to generalize to real-world populations. De-identified datasets, while preserving clinical relevancy, risk re-identification through adversarial techniques \cite{Murdoch2021_privacy_concerns}. Additionally, over 89\% of patients oppose sharing their data for secondary use \cite{Murdoch2021_privacy_concerns}, further complicating dataset generation.

% While there have been calls to share public data \cite{doi:10.1126/science.aaw1280_call_to_making_data_public}, resolving reproducibility issues with models trained on private data by large well-known institutions is practically infeasible for the average AI4H researcher from a legal and time perspective. To gauge the relevance of this problem, 

We analyzed mentions of well-known public dataset repositories in AI4H conferences and PubMed papers to estimate public dataset usage (Figure \ref{fig:data_trends}). It is important to note that this is a proxy measure and may not perfectly capture actual usage. Mentioning a public dataset name does not necessarily imply its use, and our approach might also overlook less well-known public datasets. The detailed validation is presented in Table \ref{tab:manual_validation}. 

Our analysis revealed several interesting trends across affiliations and topics. 
Figure~\ref{fig:data_trends}(a) confirmed that private datasets consistently dominate, accounting for roughly 65-75\% of all dataset usage from 2018 to 2024.
It also shows that 
those specialized AI healthcare conferences (CHIL, ML4H, and MLHC) tend to use more public datasets (about 60-70\%) compared to general medical literature in PubMed (only 25\%), suggesting these AI4H conferences might place greater emphasis on reproducibility and open science practices. %The prevalence of public dataset usage varied across conferences, with CHIL showing the highest rate of mentions (up to 71\%, Figure \ref{fig:data_trends}a). 
This variance highlights the different data usage and sharing approaches within the AI4H community. Further details about the public datasets discussed in this analysis can be found in Appendix \ref{apd:public_dataset}.

As shown in Figure~\ref{fig:data_trends}(b-c), Biosignal papers contained the largest proportion of public dataset mentions, while papers authored solely by industry organizations mentioned public datasets more frequently than their academic or mixed counterparts. This surprising finding may be attributed to our classification of research hospitals as academic institutions, which are more likely to have access to private patient data than companies.

Another notable observation (Figure~\ref{fig:data_trends}(d-e)) was the correlation between public dataset mentions and higher citation counts, suggesting potential benefits for leveraging public datasets (t-test $p < 0.05$ in Figure \ref{fig:data_trends}e). 

% Most research papers tend to rely on private datasets, which can make reproducibility expensive and difficult. However, many papers reference public datasets, \rev{making direct reproducibility feasible.} Later, we will explore potential solutions to these challenges, aiming to enhance reproducibility and transparency in AI4H research.

\subsection{Proprietary Code}
\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{figs/CodeSharingReproducibility.drawio.png}
    \caption{ Trends in Code Sharing: (a) Code-sharing percentage across different venues over time. Conference papers share code significantly more often than other PubMed papers. (b) Rate of code sharing by topic: Biomedicine papers share code slightly more often. (c) Rate of code sharing by affiliation: Industry shares slightly less than others. (d) Distribution of citation counts for papers with and without code over time: Papers that share code generally have at least the same number of citations or more each year. Citation counts are limited to 50 or below to better visualize typical citation numbers beyond outlier papers. (e) Cumulative distribution of code sharing vs. no code sharing: Papers that share code overall have more citations, regardless of outlier status.}
    % \vspace{-0.6cm}
    \label{fig:code_trends}
\end{figure}
Proprietary code in AI4H significantly hinders reproducibility. Many models use undisclosed proprietary algorithms, compromising transparency and patient safety in healthcare. A critical review \cite{Haibe-Kains2020_rebuttal_to_Google_nature_paper_with_no_code_no_data} of Google's breast cancer detection paper \cite{McKinney2020_google_breast_cancer_detection} highlights this issue, noting that insufficient details and lack of code make the high-impact work irreproducible.

To assess code-sharing trends, we tracked the presence of GitHub, Zenodo, GitLab, or Colab links within the main text as an upper-bound proxy of technical reproducibility, acknowledging that linked code may not always be complete, runnable, correctly implemented, or related to the described method. 

Figure \ref{fig:code_trends}(a) reveals increased code-sharing over time for conference venues but little change for PubMed articles (less than 20\% with code repository in their papers). CHIL and ML4H demonstrate higher rates of code mentions than MLHC, possibly due to stricter sharing requirements. However, at least 58\% of recent MLHC papers still do not share code within their main text, while PubMed's substantially lower code-sharing rate indicates that technical reproducibility remains a significant concern in AI4H. 

Figure \ref{fig:code_trends}(b-c) shows that most papers, regardless of topic or affiliation, do not share their code. Notably, industry affiliations share code slightly less often than mixed or academic affiliations. Interestingly, AI papers related to biomedicine (such as those focused on genomics) tend to share code more, while electronic health record-related (EHR) papers share code the least. 

Figure \ref{fig:code_trends}(d-e) confirmed that sharing code, similar to mentioning datasets, correlates with higher citation counts in the future. However, the significant overlap in these distributions indicates that individual academics may not notice a meaningful difference, even though a statistically significant difference exists (t-test $p < 0.05$) in Figure \ref{fig:code_trends}(e).

\subsection{Lack of Standardization in Data Processing Pipelines}
The limited standardized data processing practices in AI4H significantly impede reproducibility. Healthcare data, especially from EHRs, demands extensive preprocessing, including cohort selection, missing data management, feature normalization, and categorical variable encoding. Without a standard framework, research teams employ diverse methods, leading to substantial variability in data processing \cite{wornow2023shaky_foundations}. This variability affects model performance, complicating cross-study comparisons and result replication. 

\rev{Furthermore, improper data handling can introduce leakage, resulting in overly optimistic model performance. 
For example, studies by Kapoor et al. \cite{kapoor2022leakagereproducibilitycrisismlbased}, Vandewiele et al. \cite{Vandewiele_2021_preterm}, and Roberts et al. \cite{Roberts2021_CovidPitfalls} reveal data leakage issues in pre-term birth prediction and COVID-19 detection models, leading to inflated performance metrics. Standardizing data processing practices is, therefore, crucial for enhancing reproducibility and ensuring the reliability of AI4H models. 
}

To promote standardization in data processing, the OHDSI community has adopted a common data model known as OMOP-CDM~\cite{noauthor_undated-mg}. This model serves as a foundation for analytic pipelines and has gained significant traction in health informatics communities. Similarly, the Medical Event Data Standard (MEDS) is another initiative aimed at standardizing data for applications that are compatible with machine learning~\cite{arnrich2024medical}. \rev{However, we note that the adoption of these standards is still incomplete.}

\subsection{\rev{Error Rates of Noisy Analysis}}
\rev{To validate our automated keyword search analysis, we manually examined 30 papers. Our code sharing detection achieved 87\% accuracy, while public dataset detection showed 77\% accuracy with 90\% precision (Table \ref{tab:manual_validation}). While our code sharing estimates align with manual validation, we likely underestimate public dataset usage due to the increase in availability of public health datasets beyond well-known repositories. However, given the high precision, this lower bound serves as a reliable worst-case metric. Additionally, we evaluated the medical frontier LLM's zero-shot topic classification performance. The results showed high accuracy, with discrepancies between manual and LLM classifications often representing equally valid alternative categorizations.}

\begin{table}[h!]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{l*{6}{c}}
\toprule
\textbf{Category} & \textbf{Accuracy} & \textbf{Precision} & \textbf{Recall} & \textbf{F1 Score} & \textbf{Estimated Rate} & \textbf{True Rate} \\
\midrule
Public Dataset Usage & 0.77 & 0.90 & 0.60 & 0.72 & 0.33 & 0.50 \\
Code Sharing & 0.87 & 0.71 & 0.71 & 0.71 & 0.23 & 0.23 \\
Topic Classification & 0.93 & 0.94 & 0.93 & 0.93 & - & - \\
\bottomrule
\end{tabular}%
}
\caption{\rev{Manual validation of our automated approach on 30 randomly sampled papers, examining code sharing, public dataset usage, and topic classification. Comparing true rates from manual review against estimated rates from keyword searches, we found exact agreement between methods for code sharing (23\% both estimated and true), while public dataset usage was significantly underestimated (33\% estimated vs 50\% true). Topic classification performed exceptionally well, while code sharing detection was reliable but conservative, and public dataset detection showed high precision but missed some instances due to varied datasets not covered in the PapersWithCode API or our initial pool of popular datasets.}}
\label{tab:manual_validation}
\end{table}






% \begin{table*}[h]
% \centering
% \begin{tabular}{l|c|c|c|c|c|c|c}
% \toprule
% \textbf{Year} & \textbf{2018} & \textbf{2019} & \textbf{2020} & \textbf{2021} & \textbf{2022} & \textbf{2023} & \textbf{2024} \\
% \midrule
% CHIL Total Papers & * & * & 23 & 27 & 24 & 41 & 40 \\
% \hline
% MLHC Total Papers & 36 & 70 & 66 & 31 & 67 & 76 & * \\
% \hline
% ML4H Total Papers & * & 18 & 25 & 19 & 31 & 41 & * \\
% \hline
% PubMed Total Papers & 379 & 602 & 1,028 & 1,994 & 3,605 & 2,277 & 93 \\
% \bottomrule
% \end{tabular}
% \caption{Total number of papers scraped from major AI4H conferences and PubMed (2018 to 2024). * denotes missing info.}
% \label{tab:total_papers}
% \vspace{-0.3cm}
% \end{table*}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=1.0\textwidth]{figs/CodeSharingLinePlot.png}
%     \caption{Trends of code sharing in major AI4H conferences and PubMed publications over time. We observe a steady increase in the overall percentage of code sharing over time.}
%     \label{fig:mlhc_code_sharing}
%     \vspace{-0.5cm}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=1.0\linewidth]{figs/ParallelCoordPlot.png}
%     \caption{Distribution of public dataset usage across different venues. The analysis reveals that MIMIC is the most frequently used public dataset in published papers.}
%     \label{fig:public_dataset_distribution}
%     \vspace{-0.4cm}
% \end{figure}
% \begin{wrapfigure}{r}{0.4\textwidth}
%     \centering
%     \vspace{-0.5cm}  % Adjust vertical spacing if necessary
%     \includegraphics[width=0.4\textwidth]{figs/ParallelCoordPlot.png}
%     \caption{Distribution of public dataset usage across different venues. The analysis reveals that MIMIC is the most frequently used public dataset in published papers.}
%     \label{fig:public_dataset_distribution}
%     \vspace{-0.4cm}  % Adjust vertical spacing if necessary
% \end{wrapfigure}


==> sections/reproducibility_existing_tools.tex <==
\section{\rev{Existing Solutions Towards Improving Reproducibility}} \label{apd: existing solutions explored}
% While we were unable to discuss alternative solutions in the main text due to brevity's sake, we discuss the drawbacks of existing reproducibility solutions here. 
\rev{To better contextualize the role of open source software and benchmarks,} we \rev{briefly} explore various \rev{existing} reproducibility solutions and their respective trade-offs below. \rev{While each have their own merits, they all have drawbacks that prevent widespread adoption from the AI4H research community.}

\subsection{\rev{Guidelines and Standards}}
Numerous reproducibility \rev{guidelines and standards} have been proposed to improve research reproducibility in healthcare \cite{kapoor2022leakagereproducibilitycrisismlbased, CLAIM_Checklist_doi:10.1148/ryai.2020200029, Collinse078378_tripod, 10.1093/jamia/ocaa088_minimar, RAHROOH2024104551_automate_meta_data_checklist_reproducibility}. These checklists serve multiple purposes, including guiding authors in sharing essential information, preventing data contamination, improving the reproducibility of shared work, and providing scoring and ranking metrics to measure a paper's reproducibility \cite{pineau2020improvingreproducibilitymachinelearning, heil2021reproducibility_gold_bronze_silver}.

While useful as preventative measures \rev{and guidelines}, checklists have notable limitations. They do not directly aid in implementing or validating methods, and users may input faulty information. Furthermore, studies by \cite{kapoor2022leakagereproducibilitycrisismlbased} and \cite{Edin_2023_med_coding_repl} show that many subsequent works reuse dataset preprocessing code from earlier studies that may not have undergone rigorous reproducibility audits.

Consequently, a significant body of work still requires manual auditing and validation. This task is becoming increasingly challenging as AI-related health publications have more than doubled between 2018 and 2021 \cite{JIMMA2023100041Bibliometric}. Our survey of released PubMed papers in Figure \ref{fig:scraping} supports this finding. As such, the next crucial step is to make it easier for researchers to adhere to reproducibility standards while ensuring thorough validation of existing work.

\subsection{\rev{Automation and Tooling}}
\rev{A range of technical tools and platforms has been developed to support reproducibility efforts, aiming to streamline workflows and enhance transparency. These tools address various aspects of the research process, from experiment tracking to model releasing. Tools like Hydra and OmegaConf enable consistent and scalable management of experimental configurations. Platforms such as Hugging Face allows efficient sharing of model checkpoints. Platforms like TensorBoard, Weights \& Biases, and Neptune provide easier management of experiments.}

\rev{While these tools significantly enhance reproducibility, they are primarily designed for general machine learning tasks and are not tailored to address the unique challenges of AI4H. They are better suited as complementary counterparts rather than direct solutions for AI4H-specific reproducibility challenges. To fully address the challenges discussed earlier, AI4H requires tools explicitly designed to cater to its unique needs.} 

% \textbf{Lightweight wrapper APIs}, such as those proposed by \cite{hartley2020dtoolai}, are easy to integrate into existing workflows and enable logging of training hyperparameters. However, they fall short of providing comprehensive reproducibility pipelines. \textbf{General machine learning platforms}, exemplified by Azure \cite{GUNDERSEN202234_ML_Platforms}, aid in enforcing some reproducibility aspects but often lack comprehensive adherence to guidelines.

% Recent innovations include the use of \textbf{Large Language Models} (LLMs) to automatically fill out reproducibility checklists \cite{10.1145/3641525.3663629_LLM_reproduc}. However, these attempts have yielded mixed results, often disagreeing with human evaluators. \textbf{Closed-end Graphical ML pipelines}, such as GalaxyML \cite{Gu2021-ut_galaxy_ml} and Simon \cite{Tomic2021-ts_SIMON}, enable users to reproduce others' work easily but restrict expressiveness, making advanced AI research challenging.

% For widespread adoption, incentives are crucial. Current solutions face various challenges. Lightweight wrappers add extra steps to potentially complex pipelines, while ML platforms may not adapt well to existing research workflows. Graphical services like GalaxyML and Simon have limited application in advanced AI4H research. LLMs face distrust due to potential hallucinations \cite{huang2023surveyhallucinationlargelanguage}.

% In conclusion, existing reproducibility solutions may not provide sufficient incentives for wider community adoption and may even indirectly discourage their use. The field requires a more balanced approach that combines ease of use with comprehensive reproducibility features while maintaining the flexibility needed for advanced research.




==> sections/reproducibility_open_source.tex <==
\input{sections/reproducibility_existing_tools}
\section{Create Open-source Software and Benchmarks for Enhancing Reproducibility in AI4H}

To address the reproducibility crisis in AI for Health (AI4H), we propose the following systematic, behavior-driven strategies. 

\subsection{Open-Source Software and Benchmarks}

The foundational step in enhancing reproducibility is making tools and standards openly accessible and visible. Promoting open science through standardized data preprocessing pipelines and diverse benchmarks highlights the importance of reproducibility. Open-source platforms enhance transparency by making code, models, and workflows publicly available, while standardized benchmarks provide consistent frameworks for evaluating model performance in clinical settings, enabling validation across studies.

For example, widely adopted libraries like PyTorch~\cite{paszke2019pytorchimperativestylehighperformance}, scikit-learn~\cite{scikit-learn}, and HuggingFace~\cite{wolf2020huggingfacestransformersstateoftheartnatural} have standardized key components of machine learning and natural language processing, thus enhancing reproducibility. 
In AI4H, open-source software like \textbf{PyHealth}~\cite{10.1145/3580305.3599178_PyHealth}, \rev{MonAI \cite{cardoso2022monaiopensourceframeworkdeep_monai},} \textbf{YAIB}~\cite{vandewater2024icubenchmarkflexiblemulticenter_YAIB}, \rev{ \textbf{RENOIR}~\cite{Barberis2024_renoir}, MEDS~\cite{arnrich2024medical} and open source initiatives like OHDSI \cite{hripcsak2015observational_ohdsi}}  become increasingly valuable for reproducibility. \rev{OHDSI has created guidelines for standardizing the format of clinical data. Open source software surrounding the standardization of publicly formatted data should not be understated.} 
\rev{For instance}, open datasets such as MIMIC~\cite{Johnson2023-MIMIC} are frequently utilized; over 28\% of ML4H papers in recent years have used MIMIC data. \rev{To better standardize the curation and accessibility of MIMIC data, open source software such as PyHealth \cite{10.1145/3580305.3599178_PyHealth}, MEDS~\cite{arnrich2024medical}, and YAIB \cite{vandewater2024icubenchmarkflexiblemulticenter_YAIB} aid in the data preprocessing of large public datasets for various downstream clinical tasks. Taking a step further, open source container systems like Docker \cite{Openja_2022_docker_practices, moreau2023containers} can dramatically reduce the lower-level system software compatibility barriers of running AI pipelines.} Clearly, promoting the availability of these resources helps researchers align on common practices, facilitating reproducibility.

\subsection{Incentivizing Reproducibility}
To encourage the widespread adoption of reproducibility practices, we must make them appealing. Open-source tools should offer benefits that outweigh any perceived burdens. Libraries like PyTorch and HuggingFace attract users through time-saving APIs, simplifying reproducibility while providing efficiency and strong community support. Recognizing and rewarding reproducible work through special publications, awards, or formal acknowledgment can further incentivize researchers. \rev{For instance, schools such as Stanford Medicine have created award programs for those who contribute greatly towards reproducible practices to further incentivize creating accessible open source software and benchmarks \cite{stanford_sporr_rare_rewards}.} Establishing systems to honor those who successfully reproduce others' work promotes a culture of verification and validation within the community.

\subsection{Lowering Barriers to Contribution}
It is crucial to simplify the adoption of reproducibility practices. Enhancing functionality of these AI4H opensource tools like PyHealth~\cite{10.1145/3580305.3599178_PyHealth}, YAIB~\cite{vandewater2024icubenchmarkflexiblemulticenter_YAIB}, and MEDS~\cite{arnrich2024medical}, improving user experience, and demonstrating their impact on research can bridge this gap.

Centralized open-source platforms and established workflows enable plug-and-play model development, allowing researchers to focus on innovative problem-solving rather than redundant preprocessing steps. Improving integration with popular programming languages like Python and expanding the range of AI4H tasks covered can make these tools more accessible to the community.

\textbf{Educational Initiatives.} Open-source software is also pivotal in teaching reproducibility in graduate-level healthcare ML courses. Institutions such as MIT \cite{mit_ocw}, Johns Hopkins \cite{jhu_ml}, Georgia Tech \cite{gatech_dl}, and University of Illinois Urbana-Champaign (UIUC) \cite{uiuc_cs598} utilize open-source tools to teach key concepts, often through project-based assignments that try to replicate published research. Incorporating reproducibility-focused projects enriches students' learning experiences and promotes reproducibility. \rev{Other non-academic educational programs exist such as the Linux Foundation's open source software development course \cite{linux_foundation_ossd} and NumFOCUS's wide array of open source educational programs \cite{numfocus}.} These projects can highlight the impact of reproducibility on career development. The resulting code repositories of reproducibility case studies can showcase reproducibility for the broader community. 

\subsection{Celebrating Success in Reproducibility}
Reinforcing reproducibility practices requires making the experience rewarding. Celebrating successes—such as accurate reproductions of studies or high-quality documentation—encourages continued commitment to reproducible methods. Public recognition, badges for reproducible publications, and journal incentives can create a positive feedback loop. Organizing events like reproducibility hackathons can gamify the process, making it enjoyable and collaborative.

\rev{\textbf{Moving Cultural Norms.} Part of making reproducibility sustainable is creating a culture where reproducible practices are naturally rewarded. While the volume of AI4H publications has grown exponentially over the past decade \cite{senthil2024bibliometric_trends_AI4H}, the prevailing "publish or perish" academic environment \cite{rawat2014publish_or_perish, stupple2019reproducibility_crisis_npj_digital} often forces researchers to prioritize publication output over reproducibility efforts. This pressure frequently results in research remaining private and inaccessible. However, successful examples of fostering reproducibility exist in adjacent fields. The Natural Language Processing (NLP) community, through open source platforms like HuggingFace \cite{wolf2020huggingfacestransformersstateoftheartnatural}, has demonstrated how reducing technical barriers to sharing models and datasets can transform research culture. Despite some technical limitations, HuggingFace has successfully created an environment where the visibility and recognition gained from sharing reproducible NLP pipelines outweigh the costs of implementing reproducible practices. For large foundational models in NLP, open source chatbot arenas \cite{chiang2024chatbotarenaopenplatform} have created leaderboards where the best models are given recognition, directly incentivizing users to use and interact with these models. This success story suggests a promising path forward for AI4H: by building sufficient software infrastructure and momentum, we can lower the barriers to sharing models and benchmarking on public datasets. A more health related example is PhysioNet \cite{PhysioNet}, which has streamlined the sharing of medical datasets and become a pillar in the sharing of the dominant MIMIC \cite{Johnson2023-MIMIC} series of datasets, commonly used across the AI4H space. While this approach may not solve all reproducibility challenges, it could significantly shift the cultural attitudes toward reproducibility in the field. }

\textbf{Reproducibility Hackathons.} 
While open-source software is essential for enabling reproducibility in research, \rev{it} can \rev{also} serve as a powerful catalyst to promote and advocate for reproducibility by significantly reducing development time~\cite{Cokelaer2023-vz_reprohackathons, bender2024libraries_CMU_reprohackathons}. In the field of healthcare AI, enhanced tools make it easier for both students and professionals to participate in \rev{hackathons}, fostering collaboration on shared datasets like MIMIC and the UK Biobank. Participants can share code and concentrate on documenting reproducible workflows, ultimately building a public repository of reproducible solutions. Offering sponsorships and prizes can enhance the experience, increase engagement, and underscore the importance of reproducibility. For example, a recent Kaggle competition on EEG classification organized by academic researchers received \$50K in sponsorship from pharmaceutical, medical device, and technology companies and attracted hundreds of submissions~\cite{UnknownUnknown-yy}.

\subsection{\rev{Enforcing Reproducible Practices}}
\rev{The ultimate goal is to encourage widespread adoption of reproducible practices across the research community. As discussed in Section \ref{sec: Crisis}, while patient privacy concerns often prevent the direct replication of study results, sharing code generally poses no privacy risks. Our analysis in Figure \ref{fig:code_trends}a reveals a notable trend: conference venues that have implemented code sharing mandates have achieved substantially higher rates of code mentions in publications. In contrast, journal publications (indexed in PubMed) have not yet widely adopted such requirements, as shown in Figure \ref{fig:code_trends}a - a gap that could be addressed through policy changes. For academic researchers, who unlike their industry counterparts are not constrained by proprietary code concerns, code sharing should be a straightforward and enforceable requirement.}

\subsection{\rev{Moving Targets of Reproducibility}}
As datasets and models evolve across environments and time, reproducibility remains a moving target in both healthcare systems and when adopting new models. Well-written open source software addresses this challenge by enabling researchers and practitioners to seamlessly integrate state-of-the-art models and retrain them on new data distributions—crucial for both research advancement and practical implementation.
While reported metrics may not reflect real-world performance on target patient populations, evaluating new models typically requires access to source code, especially when training details are vaguely described in the literature. Transparent public benchmarks become especially valuable as training costs grow prohibitively expensive, as with LLMs \cite{zhao2023surveylargelanguagemodels}, allowing practitioners to reference established metrics before investing in adaptation to private data.
Although sensitive patient data in healthcare settings must remain protected due to privacy regulations, publicly available code simplifies model adaptation to these privacy-sensitive target distributions. Moreover, open-source software directly addresses the challenge of shifting distributions over time. By enabling evaluation of published models on specific cohorts across time periods, it facilitates explorations in conceptual reproducibility—determining whether one model consistently outperforms another across changing domains. Ultimately, methods lacking publicly available, well-documented code are frequently overlooked or avoided by healthcare practitioners, regardless of their potential benefits, as implementation risks outweigh theoretical advantages.

\subsection{\rev{The Future of Reproducibility with Open Source Software and AI Agents}}
\rev{While Large Language Models (LLMs) alone may not be reliable judges of reproducibility \cite{10.1145/3641525.3663629_LLM_reproduc}, they demonstrate remarkable capabilities when integrated with tools and programmatic APIs as agents \cite{li2024reviewprominentparadigmsllmbased_tool_agents, yang2024llmwizardcodewand}. These AI agents have shown proficiency in diverse healthcare tasks, from reasoning over electronic health records \cite{shi2024ehragentcodeempowerslarge_EHR_agent} to conducting data analysis \cite{wuehrflow} using existing open source software tools. The development of more robust open source software tools for healthcare model deployment and public dataset access could significantly enhance these LLM agents' capabilities. Such tools would enable AI agents to more effectively reproduce and prototype AI pipelines for healthcare data. This technological advancement could provide a scalable solution to the growing challenge of reproducing results from the exponentially increasing number of AI4H publications.}



% \section{Open Source Software and Benchmarks for Improving Reproducibility}
% Addressing the reproducibility crisis in AI4H requires a multi-faceted approach, including promoting open science practices, establishing standardized data preprocessing pipelines, and developing diverse benchmarks. A key component is the development and adoption of open-source software and benchmarks. Open-source platforms enhance transparency and reproducibility by making code, models, and data preprocessing workflows publicly accessible. Robust benchmarks, in turn, provide a consistent framework for evaluating model performance in real-world clinical settings, ensuring that research outcomes can be consistently validated across studies.

% For widespread adoption of reproducibility-enhancing software, immediate incentives must outweigh the initial cost of time and extra effort. Widely adopted libraries like PyTorch \cite{paszke2019pytorchimperativestylehighperformance}, scikit-learn \cite{scikit-learn}, and HuggingFace \cite{wolf2020huggingfacestransformersstateoftheartnatural} have reduced technical reproducibility issues by standardizing machine learning and NLP development. These packages offer clear incentives, such as time-saving APIs, which improve reproducibility without requiring significant effort to adopt.

% In the AI4H domain, a significant proportion of medical AI research consistently utilizes common large datasets, such as the Medical Information Mart for Intensive Care (MIMIC) \cite{Johnson2023-MIMIC}. As shown in Figure \ref{fig:data_trends}, over 28\% of papers accepted to ML4H in the past five years mention MIMIC in their main text, aligning with findings from \cite{mcdermott2019reproducibilitymachinelearninghealthcrisis}. This trend suggests that while task-specific details may vary, many researchers perform similar initial processing steps using data from the same source. 

% Open-source tools like \textbf{PyHealth} \cite{10.1145/3580305.3599178_PyHealth}, \textbf{YAIB} \cite{vandewater2024icubenchmarkflexiblemulticenter_YAIB}, and \textbf{RENOIR} \cite{Barberis2024_renoir} have advanced reproducibility in AI4H, but are not yet comprehensive enough for widespread adoption. This adoption gap is evident when comparing PyHealth, the most widely-used AI4H framework, with only 965 GitHub stars, to PyTorch's 80,000+ stars. This disparity exceeds what would be expected from the difference in research volume between the fields (approximately 20,000 papers in health informatics versus 180,000 in machine learning, based on Google Scholar metrics). Each tool has limitations, such as task coverage or Python integration, particularly given Python’s dominance in AI development \cite{zhao2023surveylargelanguagemodels}.

% Despite these gaps, these libraries streamline model reproduction and standardize dataset processing, reducing risks like data leakage \cite{kapoor2022leakagereproducibilitycrisismlbased}. Centralized open-source platforms ease model development, encourage iterative improvements, and support organized reproducibility efforts into clinical AI research.

% \textbf{Reproducibility Hackathons.} Open-source software has revolutionized reproducibility hackathons, dramatically reducing development time \cite{Cokelaer2023-vz_reprohackathons, bender2024libraries_CMU_reprohackathons}. In healthcare AI, improved tools would enable students to tackle predefined tasks using public datasets like MIMIC or UK Biobank. Participants could share code openly, focusing on reproducible pipelines and clear documentation. These events would promote public dataset use, establish best practices in code sharing, and build a library of reproducible solutions for common healthcare AI tasks. By having multiple groups reproduce the same work, hackathons could highlight data preprocessing challenges and foster discussions on dataset-specific standardization.

% \textbf{Course Projects on Reproducibility.} Open-source software is crucial for teaching reproducibility in graduate-level healthcare ML courses. Programs at MIT, Johns Hopkins, Georgia Tech, and UIUC often use tools like PyTorch to teach fundamental concepts and include projects where students replicate results from published healthcare AI papers. Enhancing existing AI4H open-source software would improve students' ability to complete these projects effectively. These efforts could create a public repository of reproducibility case studies, providing a valuable resource for the broader healthcare AI community.

\section{Conclusion}
The reproducibility crisis in AI for Healthcare urgently demands attention due to its direct impact on human lives. Our analysis reveals significant challenges: 74\% of AI4H papers analyzed in this paper rely on private datasets or do not share code, and data processing lacks standardization. Although \rev{rare}, papers that use public datasets and share code tend to receive more citations, indicating that embracing reproducible practices correlates with greater research impact.

% To address these issues, we advocate for a shift toward open-source development in AI4H by:
% \begin{itemize}
%     \item Developing and extending open-source research tools to cover more clinical tasks;
%     \item Developing and promoting standardized preprocessing pipelines across healthcare datasets;
%     \item Creating robust benchmarks for meaningful AI4H model comparison;
%     \item Fostering collaboration between computer scientists and healthcare professionals;
% \end{itemize}
The general machine learning community has embraced open-source practices for over a decade, and it is crucial for AI in health (AI4H) to do the same due to the high stakes involved. By prioritizing open-source development, we can enhance reproducibility, accelerate progress, and enable researchers to concentrate on innovation instead of repeatedly developing data processing steps. This shift will foster trust in AI healthcare solutions by promoting transparency, which is essential for safe and effective deployment in clinical settings. The future of AI in healthcare relies not only on breakthroughs but also on our ability to validate, reproduce, and implement innovations safely in real-world practice.

%Realizing this potential requires expanding existing packages like PyHealth to cover more clinical tasks, promoting inherently reproducible practices. The general ML community has advocated for this approach for over a decade; it is time for AI4H to follow suit. Given the high stakes in healthcare AI, reproducibility and transparency are crucial for public health and safety. We urge the AI4H community to prioritize open-source tool development and adoption. This will enhance study reproducibility and accelerate field progress. By leveraging a standardized codebase, researchers can focus on innovative algorithms and clinical applications rather than reinventing foundational steps. Moreover, open-source practices can foster collaboration between computer scientists and healthcare professionals, leading to more impactful AI solutions.

% As we stand at the cusp of a new era in healthcare, where AI promises to revolutionize patient care, diagnosis, and treatment, ensuring the reliability and reproducibility of our methods is paramount. The development and widespread adoption of comprehensive open-source software in AI4H is not just a technical necessity, but a ethical imperative that will shape the future of healthcare technology.



% Despite papers with public datasets tending to share code at higher rates, Figure \ref{fig:mlhc_data_code} reveals that large proportions (upwards of 76 \% on PubMed) of papers using publicly accessible medical datasets do not share code despite the potential for code reuse across works.
% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figs/PublicPrivateBar.png}
%     \caption{Papers with public datasets tend to share more code links. However, large proportions of papers mentioning public datasets still do not share code.}
%     \label{fig:mlhc_data_code}
% \end{figure} % for john: remove yearly dimension, and just plot the overall per venue.
